Convergence in a Repeated Non-atomic Routing Game with Partial Signaling

We study the following repeated non-atomic routing game. In every round, nature chooses a state in an i.i.d. manner according to a publicly known distribution, which influences link latency functions. The system planner makes private route recommendations to participating agents, which constitute a fixed fraction, according to a publicly known signaling strategy. The participating agents choose between obeying or not obeying the recommendation according to cumulative regret of the participating agent population in the previous round. The non-participating agents choose route according to myopic best response to a calibrated forecast of the routing decisions of the participating agents. We show that, for parallel networks, if the planner's signal strategy satisfies the obedience condition, then, almost surely, the link flows are asymptotically consistent with the Bayes correlated equilibrium induced by the signaling strategy.

==> Convergence in a Repeated Non-atomic Routing Game with Partial Signaling/abstract.tex <==
\begin{abstract}
We study the following repeated non-atomic routing game. In every round, nature chooses a state in an i.i.d. manner according to a publicly known distribution, which influences link latency functions. The system planner makes private route recommendations to participating agents, which constitute a fixed fraction, according to a publicly known signaling strategy. The participating agents choose between obeying or not obeying the recommendation according to cumulative regret of the participating agent population in the previous round. The non-participating agents choose route according to myopic best response to a calibrated forecast of the routing decisions of the participating agents. We show that, for parallel networks, if the planner's signal strategy satisfies the obedience condition, then, almost surely, the link flows are asymptotically consistent with the Bayes correlated equilibrium induced by the signaling strategy.  
\end{abstract}

==> Convergence in a Repeated Non-atomic Routing Game with Partial Signaling/calibrated-forecast.tex <==
\subsection{Connection to Calibrated Forecast}
\label{sec:forecast}
\cite{Foster.Vohra:97} studies a two player repeated game, in which, in each round, each player forecasts the probability $p=(p_1,\ldots,p_{\nlinks})$ of decisions for the other player. Convergence to the set of correlated equilibria is established if the forecasting rule is \emph{calibrated}. Let $N(p,k)$ be the number of rounds up to the $k$-th round in which the forecast is $p$, and let $\rho(p,j,k)$ be the fraction of these rounds for which the other player plays $j$. Then the forecasting rule is said to be calibrated if:
\begin{equation}
\label{eq:calibration-original}
\lim_{k \to \infty} \sum_p \Big|\rho(p,j,k)-p_j\Big| \frac{N(p,k)}{k} = 0 \qquad \forall \, j
\end{equation}

In contrast to \cite{Foster.Vohra:97}, our setting considers non-atomic agents, and the utility of every player depends also on the state $\state$, which changes from one round to the next. Non-atomicity gives $B$ agents sufficient samples to compare forecast with outcome on a per round basis. Specifically, the flow forecast $\hat{x}_j$ (after normalization by $\pfrac$) could be interpreted as the forecast of the probability with which an individual $P$-agent will pick route $j$, and similarly $x_j$ is the probability with which a $P$-agent actually picks $j$. Therefore, a reasonable adaptation of \eqref{eq:calibration-original} to our setting is that the $B$ agents' forecast is calibrated if: 
%
%However, different realizations of $\state$ in different rounds suggests the following alternative to \eqref{eq:calibration-original}. Let $\tilde{N}(\state,k)$ be the number of rounds up to the $k$-th round in which the state realization is $\state$. We shall call the $B$ agents' forecast to be calibrated if
%\begin{equation*}
%\label{eq:calibration-modified}
%\lim_{k \to \infty} \sum_{\state \in \allstates}
%\end{equation*}
%
%Therefore, the forecasting rule is called calibrated in our non-atomic setting if:
\begin{equation}
\label{eq:calibration-modified}
\lim_{k \to \infty} \frac{1}{k} \sum_{t=1}^k \Big|x_j(t) - \hat{x}_j(t) \Big| = 0 \qquad \forall \, j
\end{equation}
for almost every i.i.d. realization of $\state(t) \sim \prior$.
%shows that in a 2-player repeated game, the limit of the sequence of plays is correlated equilibrium if each player uses a calibrated forecast of the other's plays and chooses the best response to the forecast distribution. In our model, $B$-agents choose the best response to their forecast of flow of $P$-agents. Naturally, we want to know if $B$-agents' method of forecasting $P$-agents' flow is calibrated in the sense of \cite{Foster.Vohra:97} subject to appropriate adaptation of our non-atomic setting.

%We can think of $B$-agents and $P$-agents as two players, and their flows over $n$ links as distribution over action set. Then the forecast $\hat{x}(\hat{\theta},\omega)$ is calibrated if
%\begin{equation*}
%\lim_{k\to \infty, \epsilon \to 0^+} \sum_{j=0}^{\lfloor \frac{1}{\epsilon} \rfloor}\frac{N(\hat{\theta}_j^{j+1},k)}{k} \int_{j\epsilon}^{(j+1)\epsilon} |\bar{x}_i(\theta, \omega_0)-\hat{x}_i(\hat{\theta},\omega_0)| d\hat{\theta}  =0, \,
%\end{equation*}
%for $\forall i \in (n), \omega_0 \in \Omega$, where $\lfloor \cdot \rfloor$ is rounding down to the nearest integer, $N(\hat{\theta}_j^{j+1},k)$ denotes the number of stages up to the $k$-th stage that $B$-agents' forecast of $\theta$ is in the interval $[j\epsilon, (j+1)\epsilon)$, $\bar{x}_i(\theta, \omega_0):= \frac{\sum_{t=1}^k \mathbbm{1}_{\hat{\theta}[t]=\hat{\theta}, \omega[t]=\omega_0} x_i(\theta(m[t]), \omega_0)}{\sum_{t=1}^k \mathbbm{1}_{\hat{\theta}[t]=\hat{\theta}, \omega[t]=\omega_0}}$, $\mathbbm{1}$ is indicator function.


Proposition~\ref{prop:gamma-lambda-non-zero} shows that $\lim_{k \to \infty} \hat{\theta}(k) - \theta(m(k))=0$. Combine with \eqref{eq:p flow dynamics-m-general-matrix} and \eqref{eq:estimated p flow dynamics-m-general-matrix}, one can easily get $\lim_{k \to \infty} x_j(k) - \hat{x}_j(k)=0$ for $\forall \, j$. Thus the forecasting rule in \eqref{eq:estimated p flow dynamics-m-general-matrix}-\eqref{eq:smoothing-model} is calibrated in the sense of \eqref{eq:calibration-modified}.


%shows that $\lim_{k \to \infty} \hat{\theta}[k] - \theta(m[k])=0$ and based on that, Theorem~\ref{prop:convergence} shows that $\lim_{k \to \infty} \theta(m[k])=0$ almost surely. Those two results implies that $\lim_{k \to \infty} \hat{\theta}[k]=0$ almost surely, which further implies that $\lim_{k \to \infty, \epsilon \to 0^+} \frac{N(\hat{\theta}_0^1,k)}{k}=1$ almost surely. For those $t$ such that $\hat{\theta}[t]\in [0, \epsilon)$, we know from proof of Theorem~\ref{prop:convergence} that $\theta(m[t])\in [0, \epsilon)$ almost surely. Thus the definition of calibrated forecast is satisfied almost surely.

==> Convergence in a Repeated Non-atomic Routing Game with Partial Signaling/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we provided convergence analysis for a non-atomic routing game with partial signaling. The decision models are reminiscent of adaptive models studied previously in the context of dynamic procedures leading to the set of correlated equilibria. Our analysis lays the foundation to extend such analysis to repeated scenarios with explicit presence of a coordinator, albeit in the context of non-atomic routing games. 

\ksmarginphantom{need to briefly discuss the challenges}
There are several natural directions for future work. We plan to extend the analysis to general increasing latency functions, and to settings involving multiple destinations. The notion of conditional universal consistency in \cite{Fudenberg.Levine:99} potentially offers a framework to unify and generalize the specific decision models of the participating and non-participating agents considered in this paper. Finally, it would be interesting to consider a multiscale routing decision framework to enable integration of traffic flow dynamics into the decision-theoretic analysis, e.g., as in \cite{Como.Savla.ea:SICON11}. 

==> Convergence in a Repeated Non-atomic Routing Game with Partial Signaling/config.tex <==
\pdfminorversion=4
\usepackage{amsmath,amssymb,bbm,color,psfrag,amsfonts,mathtools}
\usepackage{dsfont}
\usepackage{graphicx,cuted}                       % \includegraphics
%\usepackage[normalem]{ulem}    
\usepackage[pdftex,pdfpagelabels,bookmarks,hyperindex,hyperfigures]{hyperref}
\usepackage{wrapfig}
\usepackage{pdfpages}
\usepackage[ruled,lined]{algorithm2e} 
\usepackage{algpseudocode}% http://ctan.org/pkg/algorithmicx
%\usepackage{algorithm}% http://ctan.org/pkg/algorithm
   \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\usepackage{accents}
\usepackage{lipsum}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{mathtools}
\usepackage{multicol}
\usepackage{paralist}   % \begin{inparaenum}[1)]
\usepackage{kbordermatrix}

%\usepackage{enumitem}
%\setlist{parsep=0pt,listparindent=\parindent}

% revision mode 
%\usepackage{changes}
%\definechangesauthor[name={Qin}, color=orange]{q}
%\setremarkmarkup{(#2)}

% table
\usepackage{booktabs}  
\usepackage{multirow}
\usepackage[normalem]{ulem}

% caption
\usepackage{caption}
\captionsetup{width=1.0\columnwidth}
\usepackage{subcaption}

\usepackage{cite}


% algorithm
%\usepackage{algorithmic}
%\usepackage{algorithm}
% theorem environment. 
%\theoremstyle{plain} 

%\newenvironment{problem}[1][htb]
%  {\renewcommand{\algorithmcfname}{Problem}% Update algorithm name
%   \begin{algorithm}[#1]%
%  }{\end{algorithm}}

\newcounter{problem}
\newenvironment{problem}[1][]
{\refstepcounter{problem} \medskip 
\noindent
\begin{tabular}{@{}p{\textwidth}} 
\\ \toprule 
 \textbf{Problem~\theproblem:}  #1 
   \\  \midrule
   }
   {\vspace{-0.6cm} \\ \bottomrule \end{tabular}  \medskip}

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{conjecture}{Conjecture}

%\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}

%\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}

% QED filled black box
\newcommand{\qedsymbol}{$\blacksquare$}

%%% Annotation
\usepackage{color}

%% new commands

\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}

% frequently used sets
\newcommand{\ones}{\mathbf 1}
%\newcommand{\real}{{\mbox{\bf R}}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\complex}{\mathbb{C}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\mc}{\mathcal}
\newcommand{\kscomment}[1]{{\color{red} #1}}
%\newcommand{\kscomment}[1]{#1}
%\newcommand{\kscommentphantom}[1]{#1}
\newcommand{\kscommentphantom}[1]{{\color{red} #1}}
\newcommand{\kscommentcancel}[1]{{\color{red} #1}}
\newcommand{\ksmargin}[1]{\marginpar{\color{red}\footnotesize [KS]:
#1}}
\newcommand{\ksmarginphantom}[1]{}

\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\setdef}[2]{\left\{#1 \; | \; #2\right\}}
\newcommand{\zerobf}{\mathbf{0}}
\newcommand{\onebf}{\mathbf{1}}
\newcommand{\until}[1]{\{1,\dots,#1\}}
\newcommand{\map}[3]{#1: #2 \rightarrow #3}
\newcommand{\ds}{\displaystyle}

\newcommand{\fr}{\nu}
\newcommand{\prb}{\mu_0}
\newcommand{\cost}{J}
\newcommand{\congfunc}{\ell}
\newcommand{\diag}{\mathbf{diag}}

\newcommand{\prior}{\mu_0}
\newcommand{\state}{\omega}
\newcommand{\allstates}{\Omega}
\newcommand{\interior}{\mathrm{int}}
\newcommand{\signal}{\pi}
\newcommand{\signalmarginal}{{\overline{\signal}}}
\newcommand{\pfrac}{\nu}
\newcommand{\simplex}{\mc P}
\newcommand{\supersimplex}{\mathbf{P}}
\newcommand{\nlinks}{n}
\newcommand{\npaths}{\nlinks}
\newcommand{\nmesgs}{m}
\newcommand{\nstates}{s}
\newcommand{\E}{\mathrm{E}}
\newcommand{\posterior}{\mu}
\newcommand{\pflowfull}{f^{P,\text{full}}}
\newcommand{\bwe}{\mc B}
\newcommand{\allcongfunc}{\mc L}
\newcommand{\congfuncallstates}{L}
\newcommand{\allsignals}{\Pi}
\newcommand{\allsignalsposterior}{\hat{\Pi}}
\newcommand{\vect}{\mathrm{vec}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\avgcongfunc}{\bar{\congfunc}}
\newcommand{\messagespace}{\mc M}
\newcommand{\rowstochastic}{\mc R}
\newcommand{\powerset}{\mathbb{P}}
\newcommand{\regret}{r}
\newcommand{\regretplain}{I}
\newcommand{\instregret}{I^{\text{inst}}}
\newcommand{\avgregret}{I^{\text{avg}}}
\newcommand{\regretmax}{I_{\max}}
\newcommand{\regretpub}{r^{\text{pub}}}
\newcommand{\pagentprob}{p}
\newcommand{\defprob}{q^{\text{def}}}
\newcommand{\actprobplain}{p^{\text{act}}}
\newcommand{\actprob}[2]{\actprobplain_{#1,#2}}
\newcommand{\de}{\mathrm{d}}
\newcommand{\pubsignal}{\signal^{\text{pub}}}

\newcommand{\sgn}{\mathrm{sgn}}

\graphicspath{{../results/} , {../../../../fig/},{../fig/}}
%\graphicspath{{../../../fig/}}

\algnewcommand{\algorithmicgoto}{\textbf{go to}}%
\algnewcommand{\Goto}[1]{\algorithmicgoto~\ref{#1}}%






==> Convergence in a Repeated Non-atomic Routing Game with Partial Signaling/convergence.tex <==
\section{Convergence Analysis and Discussion}
\label{sec:convergence}
We shall establish convergence of \eqref{eq:instant}-\eqref{eq:smoothing-model} for $\signal$ which are \emph{obedient}, i.e., for which there exists $y \in \simplex_{\nlinks}(1-\pfrac)$ such that: 
%to the \emph{Bayes Correlated Equilibrium}~\cite{Bergemann.Morris:16} induced by $\signal$, i.e., $(\signal,y \in \simplex_{\nlinks}(1-\pfrac))$ satisfying the following:
\input{correlated-equilibrium}

Following \cite{Bergemann.Morris:16},  $(\signal,y)$ is therefore the \emph{Bayes Correlated Equilibrium} induced by $\signal$. We start the convergence analysis by considering the extreme case when there are no B-agents, i.e., when $\pfrac=1$.
\begin{proposition}
\label{prop:homo}
Consider the dynamics in \eqref{eq:instant}-\eqref{eq:p flow dynamics-m-general-matrix} with $\nu=1$, and general polynomial latency functions in \eqref{eq:polynomial-latency-function}. For any $\prb$, obedient $\pi$, and every $m(1) \in [-m_{\max},+m_{\max}]$, we have that, almost surely
$$
\lim_{k \rightarrow \infty} x_i(k) - \pi_{\omega(k),i} = 0, \qquad i \in [n]
$$
\end{proposition}

Towards consideration of the general case of heterogeneous population, we first provide an analysis of the case in the absence of the aggregator, i.e., for some fixed $m(k) \equiv m$.

\begin{proposition}
\label{prop:convergence-lambda-zero}
Consider the dynamics in \eqref{eq:instant}-\eqref{eq:smoothing-model} for some fixed $m(k) \equiv m \in [-m_{\max},+m_{\max}]$. For any $\mu_0$, obedient $\pi$, $\nu \in (0,1)$, $\hat{\theta}(1) \in [0,1]$, we have that
\begin{equation*}
\lim_{k \to \infty} \hat{\theta}(k) = \theta(m)
\end{equation*}
\end{proposition}

Next, we extend the analysis to the case when $m(k)$ evolves according to \eqref{eq:instant}-\eqref{eq:S-agent-update}.
\begin{proposition}
\label{prop:gamma-lambda-non-zero}
Consider the dynamics in \eqref{eq:instant}-\eqref{eq:smoothing-model}. For any $\mu_0$, obedient $\pi$, $\nu \in (0,1)$, $\hat{\theta}(1) \in [0,1]$, $m(1) \in [-m_{\max},+m_{\max}]$, we have that
\begin{equation*}
\lim_{k \to \infty} \hat{\theta}(k) - \theta(m(k))=0
\end{equation*}
\end{proposition}

The following results will be useful in proving convergence of link-wise flows. 

\begin{lemma}
\label{lemma:convergence}
Consider the dynamics in \eqref{eq:instant}-\eqref{eq:smoothing-model} for general polynomial latency functions in \eqref{eq:polynomial-latency-function}. For any $\mu_0$, obedient $\pi$, $\nu \in (0,1)$, and initial conditions $\hat{\theta}(1) \in [0,1]$ and $m(1) \in [-m_{\max},+m_{\max}]$, there exists a subsequence $\{m(k_s)\}_s$, whose limit is negative almost surely.
\end{lemma}

\begin{lemma}
\label{lemma:lipschitz}
The mapping $y(\theta): [0,1] \rightarrow \simplex_n(1-\pfrac)$ defined in \eqref{eq:BWE} for general polynomial latency functions in \eqref{eq:polynomial-latency-function} is Lipschitz continuous.
\end{lemma}

We are now ready to state the main result. 

\ksmarginphantom{shouldn't this theorem be about the total flow?}
\begin{theorem}
\label{prop:convergence}
Consider the dynamics in \eqref{eq:instant}-\eqref{eq:smoothing-model} for general polynomial latency functions in \eqref{eq:polynomial-latency-function}. For any $\mu_0$, obedient $\pi$, $\nu \in (0,1)$, and initial conditions $\hat{\theta}(1) \in [0,1]$ and $m(1) \in [-m_{\max},+m_{\max}]$,
we have that, almost surely
$$
\lim_{k \rightarrow \infty} x_i(k) - \nu \pi_{\omega(k),i} = 0, \qquad i \in [n]
$$
\end{theorem}


==> Convergence in a Repeated Non-atomic Routing Game with Partial Signaling/correlated-equilibrium.tex <==
%\subsection{Partial Information Correlated Equilibrium}
%\ksmargin{this definition needs work}
%The partial information correlated equilibrium induced by a signal $\pi$ is the joint distribution $\tilde{\pi}$ satisfying the following:
\begin{subequations}
\label{eq:obedience-hetero-v1}
\begin{align}
\sum_{\state \in \Omega} \ell_{\omega,i}(\signal_{\state,i} + y_i) \, \signal_{\state,i} \, \prior(\state) & \leq \sum_{\state \in \Omega}  \ell_{\omega,j}(\signal_{\state,j} + y_j) \, \signal_{\state,i} \, \prior(\state), \quad i, j \in [\npaths] 
\label{eq:obedience-hetero-v1:obedience} \\
\sum_{\state \in \Omega}  \ell_{\omega,i}(\signal_{\state,i} + y_i) \, y_i \, \prior(\state) &
\leq \sum_{\state \in \Omega} \ell_{\omega,j}(\signal_{\state,j} + y_j) \, y_i \, \prior(\state), \quad i, \, j \in [\npaths] 
\label{eq:obedience-hetero-v1:nash}
\end{align}
\end{subequations}


==> Convergence in a Repeated Non-atomic Routing Game with Partial Signaling/dynamics.tex <==
\subsection{Repeated Game Setting}
\ksmarginphantom{what is the correct terminology: repeated game or multi-stage game?}
Consider the following repeated game setting. The strategy space of a participating agent (P-agent) is $\{\mathrm{obey}, \\ \mathrm{do \, not \, obey}\}$, whereas the strategy space of a non-participating Bayesian agent (B-agent) is $\{1, \ldots, \npaths\}$. The $\mathrm{do \, not \, obey}$ behavior of the P-agents is modeled by the row-stochastic matrix $P$ with zeros on the diagonal, where $P_{ij}$ is the fraction of $\mathrm{do \, not \, obey }$ P-agents who are recommended $i$ but choose $j$. The choice of a P-agent is driven by a notion of regret, and the decision of a B-agent is myopic best response to a forecast of P-agent decisions. The details are as follows. 
% 
%
%We now postulate a discrete-time dynamical system, whose time epochs correspond to the game stages. The state of this dynamical system is the mistrust at the end of stage $k$, denoted as $m(k)$. 
%
%Let the \emph{baseline} route choice of $P$-agents be modeled by the probability vector $p$, i.e., $p_i$ denotes the fraction of $P$-agents who choose route $i$ before the introduction of the information design system. $p$ will naturally influence the route choice of those P-agents who do not trust the recommendations from the information design system once it is introduced. In order to explicitly capture the aversion to follow the recommendation, one can add granularity and model the route choice of P-agents by the row-stochastic matrix $P$ with zeros on the diagonal. Specifically, $P_{i,j}$ denotes the fraction of P-agents who receive recommendation to take route $i$, do not follow the recommendation and rather choose route $j$. 
%
%The dynamics is determined by decision models for P-, B-, and S-agents, which we describe in the next subsections.

\subsubsection{Route choice model for P-agents}
\label{sec:P-dynamic}
The outline of the decision making process of P-agents is as follows. 
At the end of stage $k$, every P-agent computes difference between the payoffs associated with the recommended choice and the alternative choice(s). These payoff differences are then aggregated over the entire population of $P$-agents to give $u(k)$. The average of the initial condition $m(1)$ and $u(1), \ldots, u(k)$, denoted as $m(k+1)$, is then mapped to regret as $\theta(m(k+1)) \in [0,1]$, which equals the fraction of P-agents who do not follow recommendation in stage $k+1$. The details for each step in this process is provided next. 

%\ksmargin{note that I changed the time index in $\theta(m(k-1))$ to be consistent with the literature; need to make such changes also in the rest of the paper}
%\kscomment{[provide details here on computation of regret for an agent who follows the recommendation, as well as for the one who does not follow]}
We assume that upon completion of the trips, all agents ($P$- and $B$-agents) have access to traffic report from the $k$-th stage. This report consists of $\omega(k)$ and $\{\ell_{\omega(k),i}\}_{i \in [n]}$. For simplicity, first consider the two-link case with $\ell_{\omega(k),1}>\ell_{\omega(k),2}$. For a $P$-agent who was recommended route 1, irrespective of whether she obeys the recommendation or not, her recommendation is sub-optimal by $\ell_{\omega(k),1}-\ell_{\omega(k),2}$. In the general case of $n \geq 2$ links, for a $P$-agent who obeys recommendation to take route $i$, the sub-optimality of the recommendation is $\congfunc_{\omega(k),i} -\sum_{j \in [n]} P_{ij} \congfunc_{\omega(k),j}$. On the other hand, for a $P$-agent who does not obey the recommendation to take route $i$ but rather takes route $j$, the sub-optimality of her recommendation is $\congfunc_{\omega(k),i} -\congfunc_{\omega(k),j}$. Taking into account the number of $P$-agents who are recommended different routes and the fraction of them who $\mathrm{obey}$ or $\mathrm{do \, not \, obey}$ the recommendation, the aggregation of payoff difference over the entire P-agent population is given by:
\begin{align}
u(k) := & \sum_{i \in [n]} \Big(\congfunc_{\omega(k),i} -\sum_{j \in [n]} P_{ij} \congfunc_{\omega(k),j} \Big) \pi_{\omega(k),i} \left(1-\theta(m(k))\right) + \sum_{i,j \in [n]} \Big(\congfunc_{\omega(k),i} - \congfunc_{\omega(k),j} \Big) P_{ij}\pi_{\omega(k),i} \theta(m(k)) \nonumber \\
=& \sum_{i,j \in [n]} \Big(\congfunc_{\omega(k),i} - \congfunc_{\omega(k),j} \Big) P_{ij} \pi_{\omega(k),i} \nonumber \\
= & {\pi_{\omega(k)}}^T (I-P) \congfunc_{\omega(k)}
\label{eq:instant} 
\end{align}
%where we have dropped the dependence of $\{\ell_{\omega,i}: i \in [n]\}$ and $\omega$ on $k$ for brevity. 
where $\congfunc_{\omega(k)}$ is the $\nlinks \times 1$ column vectors whose entries are $\congfunc_{\omega(k),i}, \, i \in [n]$.
%In the spirit of transparency, we assume that the the structure of the dynamics in \eqref{eq:S-agent-update} is known to the B-agents. 
The average of these instantaneous payoff differences (as well as the initial condition $m(1)$) is:
\begin{equation}
\label{eq:S-agent-update}
\begin{split}
m(k+1) & = \frac{1}{k+1} \left(m(1)+u(1) + \ldots u(k) \right)
\\
& = \frac{k}{k+1} m(k) + \frac{1}{k+1} u(k)
\end{split}
\end{equation}

We adopt the following notion of regret:
\begin{equation}
\label{eq:rating-to-mistrust}
\theta(m(k))=\frac{[m(k)]^+}{m_{\max}}
\end{equation}
where $m_{\max}$ is chosen to be sufficiently large so that $\theta(m(k)) \in [0,1]$ for all possible values of $m(k)$. Since $[m(k)]^+$ can be upper bounded by $\sum_{i \in [n]} \sum_{ d=0}^D \max_{\omega \in \Omega} \alpha_{d,\omega,i}$, it can then serve as a lower bound for $m_{\max}$.

$\theta(k) = \theta(m(k))$ is interpreted as the fraction of agents who do not follow recommendation. 
Therefore, the link flows induced by $P$-agents be given by: \ksmarginphantom{need more details for \eqref{eq:p flow dynamics-m-general}}
\begin{equation*}
\label{eq:p flow dynamics-m-general}
\begin{split}
x_i(k) = x_i(m(k),\omega(k)) = \pfrac \pi_{\omega(k),i} \left(1-\theta(m(k))\right) + \pfrac \sum_{j \in [n]} P_{ji} \pi_{\omega(k),j} \theta(m(k))
\end{split}
\end{equation*}
which in matrix form becomes:
\begin{align}
%\label{eq:p flow dynamics-m-general-matrix}
%\begin{split}
x(k) = x(m(k),\omega(k)) & = \pfrac \pi_{\omega(k)} \left(1-\theta(m(k))\right) + \pfrac \sum_{j \in [n]} P_{ji} \pi_{\omega(k),j} \theta(m(k)) \nonumber \\
& = \pfrac \left(\pi^{\omega(k)} - \theta(m(k)) \pi^{\omega(k)} + \theta(m(k)) P^T \pi_{\omega(k)} \right) \nonumber \\
& = \pfrac \pi_{\omega(k)} + \pfrac \theta(m(k)) (P^T - I ) \pi_{\omega(k)}
\label{eq:p flow dynamics-m-general-matrix}
%\end{split}
\end{align}
where $x(m(k),\omega(k))  \in \simplex_{\nlinks}(\pfrac)$.

\begin{remark}
The framework in \eqref{eq:instant}-\eqref{eq:p flow dynamics-m-general-matrix} is reminiscent of the \emph{regret matching} framework of \cite{Hart.Mas-Colell:00}. Details on comparison are provided in Section~\ref{sec:regret}. A few points are worth special emphasis:
\begin{enumerate}
\item The aggregation of payoff difference over all $P$-agents in \eqref{eq:instant} is inspired by platforms such as Yelp. 
\item In the framework of \cite{Hart.Mas-Colell:00}, $[m]^+$ is referred to as regret and $m_{\max}$ is the inertia parameter which captures the propensity of a $P$-agent to stick to the action choice in the previous round. On the other hand, in our setup, $\theta=[m]^+/m_{\max}$ is interpreted as the degree of obedience of an individual agent,  tuned by the parameter $m_{\max}$.
\end{enumerate}
\end{remark}

\subsubsection{Route choice model for B-agents}
The B-agents forecast the flow induced by P-agents for different realizations of $\omega$ 
using a model structurally similar to \eqref{eq:p flow dynamics-m-general-matrix}, as follows:
\begin{equation*}
\label{eq:estimated p flow dynamics-m-general}
\begin{aligned}
\hat{x}_i(k) = \hat{x}_i(\hat{\theta}(k),\omega(k)) = \pfrac \pi_{\omega(k),i} \left(1-\hat{\theta}(k)\right) + \pfrac \sum_{j \in [n]} P_{ji} \pi_{\omega(k),j} \hat{\theta}(k)
\end{aligned}
\end{equation*} 
or in matrix form as:
\begin{equation}
\label{eq:estimated p flow dynamics-m-general-matrix}
\hat{x}(k) = \hat{x}(\hat{\theta}(k),\omega(k)) = \pfrac \pi_{\omega(k)} + \pfrac \hat{\theta}(k) (P^T - I ) \pi_{\omega(k)}
\end{equation}
where $\hat{\theta}$ is B-agents' forecast of $\theta$, $\hat{x}(k)  \in \simplex_{\nlinks}(\pfrac)$. The \emph{simple} exponential smoothing model for this forecast can be written in the following equivalent forms:
\begin{align}
\hat{\theta}(k+1)& = \beta(k+1) \theta(k) + (1-\beta(k+1)) \hat{\theta}(k) \nonumber \\
 & = \hat{\theta}(k)+\beta(k+1) e_{\theta}(k) \label{eq:smoothing-model}
%& = \sum_{t=1}^k \beta(k)(1-\beta(k))^{k-t} \theta(k-1) \nonumber
\end{align}
where $e_{\theta}(k):=\theta(k)-\hat{\theta}(k)$, $\beta(k+1) \in (\beta_{\min},\beta_{\max}) \subset (0,1)$ is the smoothing parameter, and $\hat{\theta}(1) \in [0,1]$ is the initial forecast. 

%In Section~\ref{sec:estimation}, we describe various models for $\hat{\theta}$. 

Let us denote the myopic best response to the forecast as $y(\hat{\theta}(k))$. For a given $\theta \in [0,1]$, $y(\theta)$ is the unique (assuming strictly increasing latency functions $\{\ell_{\omega,i}\}_{\omega,i}$, more details in Lemma~\ref{lemma:lipschitz}) $y \in \simplex_n(1-\pfrac)$ satisfying:
\begin{equation}
\label{eq:BWE}
\begin{split}
y_i & > 0 \implies 
\\
& E_{\omega \sim \prior}[\congfunc_{\omega,i}(\hat{x}_i(\theta,\omega)+y_i)] \leq E_{\omega \sim \prior}[\congfunc_{\omega,j}(\hat{x}_j(\theta,\omega)+ y_j)], \qquad i, j \in [n]
\end{split}
\end{equation}

\begin{remark}
\label{rem:B-forecast}
Implementation of \eqref{eq:smoothing-model} requires B-agents to have access to $\theta(k)$. As we assumed in Section~\ref{sec:P-dynamic}, $B$-agents have access to state $\omega(k)$, delays $\{\ell_{\omega(k),i}\}_{i \in [n]}$. B-agents also know the fixed signal $\pi$, as well as explicit form of latency functions. For a given $\hat{\theta}(k)$, \eqref{eq:estimated p flow dynamics-m-general-matrix} gives $\hat{x}_i(k)$. \eqref{eq:BWE} then gives $y(\hat{\theta}(k))$, i.e., the flow induced by $B$-agents is known to them. Assuming the latency functions are strictly increasing, the total link-wise flows can be inferred from other information known to $B$-agents. They can then infer the actual inflows induced by $P$-agents. Using the inverse of \eqref{eq:p flow dynamics-m-general-matrix}, $B$-agents can then get $\theta(k)$. 
\end{remark}

An equivalent variational inequality characterization of $y(\theta)$ is that it is the unique $y \in \simplex_n(1-\pfrac)$ satisfying
\begin{equation}
\label{eq:BEW-VI}
\sum_{i \in [n]} \, E_{\omega \sim \prior}[\congfunc_{\omega,i}(\hat{x}_i(\theta,\omega)+y_i)] (z_i - y_i) \geq 0 \qquad \forall \, z \in \simplex_n(1-\pfrac)
\end{equation}
%In matrix form, $y(\theta)$ satisfies:
%\begin{equation}
%\label{eq:BEW-VI-matrix}
%E_{\omega \sim \prior} \, \left[ (z-y(\theta))^T \, (\alpha_0^{\omega} + \diag(\alpha_1^{\omega}) \, (\pfrac \signal^{\omega} + \pfrac \theta (P^T -I) \pi^{\omega} + y(\theta)))\right] \geq 0 \qquad \forall \, z \in \simplex(1-\pfrac)
%\end{equation}

In matrix form, $y(\theta)$ satisfies:
\begin{equation}
\label{eq:BEW-VI-matrix}
E_{\omega \sim \prior} \, \left[ (z-y(\theta))^T \, \congfunc_{\omega}(\hat{x}(\theta,\omega)+y)\right] \geq 0 \qquad \forall \, z \in \simplex(1-\pfrac)
\end{equation}

Note that the total link flow forecasted by B-agents is $\hat{x}(\hat{\theta}(k),\omega(k))+y(\hat{\theta}(k))$, but the actual flow is $x(m(k),\omega(k))+y(\hat{\theta}(k))$.


\begin{remark}
\label{rem:BWE-lipschitz}
\begin{enumerate}
\item One can show that the map defined in \eqref{eq:BWE} is Lipschitz continuous. Detailed proof in Lemma~\ref{lemma:lipschitz}. 
\item The forecast and best response combination of $B$ agent decisions is reminiscent of \cite{Foster.Vohra:97}, where convergence is established to correlated equilibrium set in two player games if the forecast is \emph{calibrated} to the plays of the opponent. We argue in Section~\ref{sec:forecast} that, with appropriate adaptation to the non-atomic setting of this paper, the forecast strategy of $B$-agents could also interpreted as being calibrated to $P$-agents' actions.  
\end{enumerate}
\end{remark}

==> Convergence in a Repeated Non-atomic Routing Game with Partial Signaling/estimation-models.tex <==
\subsection{Estimation Models for B-agents}
\label{sec:estimation}
We consider two classes of models for B-agents, inspired by Luenberger observer and exponential smoothing forecasting. 

\subsection{Luenberger-like estimation model}
In \eqref{eq:S-agent-update}-\eqref{eq:p flow dynamics-m-general}, one can interpret $m[k]$ as the state and $u[k]$ as the input driven by the output consisting of link latencies $\ell[k]=\{\ell_i^{\omega[k]}(x_i[k]+y_i[k]): \, i \in (n)\}$. The corresponding Luenberger-like observer therefore is:
\begin{equation}
\label{eq:luenberger-dynamics}
\hat{m}[k+1]=\frac{k}{k+1} \hat{m}[k] + \frac{1}{k+1} u[k] + L \left(\ell[k] - \hat{\ell}[k] \right)
\end{equation}
where $L$ is observer gain, and $\hat{\ell}[k]=\ell^{\omega[k]}\left(\hat{x}[k]+y[k]\right)$ is the estimated output. The estimation error is $e_m[k]:=m[k]-\hat{m}[k]$. The error dynamics is therefore
\begin{equation}
\label{eq:error-dynamics-luenberger}
e_m[k+1]=\frac{k}{k+1} e_m[k]- L \big(\ell[k]-\hat{\ell}[k]\big)
\end{equation}

\begin{proposition}
For every $m[1]$ and $\hat{m}[1]$, under \eqref{eq:error-dynamics-luenberger} with $L=0$, $\lim_{k \to \infty} e_m[k]=0$.
\end{proposition}
\begin{proof}
\eqref{eq:S-agent-update} can be rewritten as $m[k+1]=\frac{m[1]+\sum_{t=1}^k u[t]}{k+1}$. Using similar rewriting of \eqref{eq:luenberger-dynamics}, we get $e_m[k]=\frac{e_m[1]}{k}$, establishing the proposition.

\end{proof}

\subsection{Exponential smoothing estimation model}
Estimates produced using exponential smoothing methods are weighted averages of past observations, with the weights decaying exponentially as the observations get older. The \emph{simple} exponential smoothing model for the B-agent can be written in the following equivalent forms:
\begin{align}
\hat{\theta}[k+1]& = \beta[k] \theta[k] + (1-\beta[k]) \hat{\theta}[k] \nonumber \\
 & = \hat{\theta}[k]+\beta[k] e_{\theta}[k] \label{eq:smoothing-model}\\
 & = \sum_{t=1}^k \beta[k](1-\beta[k])^{k-t} \theta[k] \nonumber
\end{align}
where $e_{\theta}[k]:=\theta[k]-\hat{\theta}[k]$, and $\beta[k] \in (\beta_{\min},\beta_{\max}) \subset (0,1)$, is the smoothing parameter. 

\kscomment{
\begin{remark}
\label{rem:BWE-lipschitz}
Implementation of \eqref{eq:smoothing-model} requires B-agents to have access to $\theta[k]$. 
\end{remark}
}



==> Convergence in a Repeated Non-atomic Routing Game with Partial Signaling/introduction.tex <==
\section{Introduction}
Optimal decision-making for agents in modern complex socio-technical systems, such as transportation, is challenging because of dynamical environments and uncertainties. Personal mobile devices
allow the agents to stay updated on the information, and even make decisions for them. This architecture also allows the possibility for \emph{information design}, whereby the source of information, say a system planner, can strategically pick what information to reveal or make direct route recommendations 
to steer the traffic flow towards optimal social state.

\ksmarginphantom{need to pick one among agent/player/driver and stick to it}
We consider a non-atomic routing game where the link latency functions are conditional on the state of the nature, e.g., whether there is a traffic incident or not. This state is generated in an i.i.d. manner from an exogenous distribution. This distribution is known publicly to all the agents, e.g., from historical data or personal experience, but the actual realization is known only to the system planner. It is therefore natural to consider that the system planner could use this informational advantage to recommend routes to the agents in order to optimize a social objective. Such a mapping from the state realization to route recommendation is referred to as signaling strategy in line with the \emph{information design} literature~\cite{Bergemann.Morris:19}. 
The recommendations would be obeyed by the agents only if, by following it, they are better off than by making decision based only on the prior distribution of the states. Such a requirement on the signaling strategy is formally referred to as \emph{obedience constraint}. 
Extension of this constraint to a multi-round setting is not clear. Specifically, how does an agent determine obedience based on the series of recommendations and payoffs that she receives, and can a static notion guarantee persistent obedience in a multi-round setting? One naive justification is that the agents follow the recommendations in every round until they have sufficient samples to empirically evaluate the obedience condition. If the strategy indeed satisfies the obedience constraint, then the agents' evaluation would be so and therefore they will continue following the recommendation subsequently. We rather consider a setting where the agents choose between obeying or not obeying recommendation in every round from the beginning. This choice is determined by the agents' regret associated with the decision in the previous round and aggregated over all other agents. 
Moreover, we also allow for partial signaling, i.e., when only a fraction of agents participate in signaling. The rest are assumed to choose routes as best response to their forecast of the link flows induced by the participating agents.  

The motivation for the setting comes from the practical consideration that agents have the discretion to use or not to use a navigation system, and if they use one, then whether to obey the recommendation or not on any given trip. It is therefore of interest to understand the long term effectiveness of a route recommendation strategy in such a setting. The feature of our model to let the decision of a participating agent depend on the \emph{collective} experience of all the participating agents in the previous rounds is inspired by platforms such as Yelp which aggregate feedback from all users to provide a single review rating which is publicly accessible. The decision models in this paper are reminiscent of well-known models studied in the context of convergence to correlated equilibrium, e.g., \cite{Foster.Vohra:97,Fudenberg.Levine:99,Hart.Mas-Colell:00}. This is not completely surprising given that the obedience constraint has been shown to be equivalent to \emph{Bayes} correlated equilibrium~\cite{Bergemann.Morris:16}. 
Specifically, a participating agent computes regret associated with the decision in the previous round in the same spirit as \cite{Hart.Mas-Colell:00}; however, its decision in the current round depends on the cumulative regret of all the participating agents, and also, the regret determines the propensity to follow the recommendation in the current round as opposed to deviating from the decision in the previous round as in \cite{Hart.Mas-Colell:00}. The model for non-participating agents to choose routes as best response to a forecast of the flow induced by the participating agents is reminiscent of \cite{Foster.Vohra:97}. 
Our main result is that, if the signaling strategy is obedient, then the non-participating agents' forecast of the link flows induced by the participating agents converges to actual induced link flows, which in turn converges to the link flows corresponding to the Bayes correlated equilibrium associated with the signaling strategy.  

%pursuing the dynamical setting comes from the practical consideration that agents have the discretion to follow or to not to follow recommendation from a navigation system at any time. This option is further facilitated by review aggregating platforms, such as Yelp, along with personal experience. The mistrust dynamics in this paper is heavily inspired by the \emph{regret}-based learning mechanism for correlated equilibria from \cite{Hart.Mas-Colell:00}. Such parallels are natural given that optimal persuasion corresponds to searching for the best among the feasible correlated equilibria. There is a subtle difference between the standard notion of regret and the notion of mistrust that we adopt, keeping in mind the context of recommendation in this paper. The two notions coincide for agents who follow the recommendation, but are negative of each other for agents who do not follow the recommendation. A central platform aggregates the individual measures of mistrust from each agent in a moving time average fashion. This aggregate system-level measure of mistrust is publicly known and the fraction of agents who do not follow the recommendation is proportional to this aggregate measure. We show that, in the homogeneous setting, almost surely, the stochastic processes corresponding to the link flows induced by the mistrust dynamics and by absolute following of the persuasion strategy by all the agents coincide asymptotically. The inequalities characterizing the incentive compatibility constraints play an important role in establishing this convergence.  
%
%Our work is related to the literature on dynamical processes leading to correlated equilibrium, e.g., see \cite{Foster.Vohra:97,Fudenberg.Levine:99,Hart.Mas-Colell:00}. 
%There are several novel contributions of the paper which are worth emphasizing. First, a well-known interpretation of correlated equilibrium is using the concept of a coordinator. However, the coordinator is absent from the repeated game settings used in the existing convergence analyses. It is perhaps for this reason that these works can establish convergence to a \emph{set} of correlated equilibria rather than to a specific equilibrium. Our setting explicitly involves the coordinator which helps to steer the convergence to a particular equilibrium. Second, a further nuance is introduced due to the partial signaling aspect, because of which the probability distribution used by the agents in the formulating the correlated equilibrium condition is not the same for every agent. 
%Third, to the best of our understand, there does not exist convergence analysis for correlated equilibria in non-atomic games. 

The rest of the paper is organized as follows. Section~\ref{sec:model} formulates the non-atomic routing game with partial signaling, defines the notion of partial information correlated equilibrium, as well as describes the repeated game setting. Section~\ref{sec:convergence} provides convergence analysis, and Section~\ref{sec:simulation} provides illustrative simulation results. Concluding remarks are provided in Section~\ref{sec:conclusion}. The proofs of all the technical results are collected in the Appendix.

We end this section by defining key notations to be used throughout this paper. Let $\triangle(X)$ denote the set of all probability distributions on $X$. 
For a vector $x \in \RR^n$, $\diag(x)$ will denote the $n \times n$ diagonal matrix with elements of $x$ on the main diagonal. 
%Let $\powerset(X)$ denote the power set of $X$. 
For an integer \( n \), we let \( [n]:= \{1, 2, \ldots, n\} \). For $\lambda \geq 0$, let $\simplex_n(\lambda):=\setdef{x \in \real_{\geq 0}^n}{\sum_{i \in [n]} x_i = \lambda}$ be the $(n-1)$-dimensional probability simplex of size $\lambda$. When $\lambda=1$, we shall simply denote the simplex as $\simplex_n$ for brevity in notation. For a real number $r \in \real$, we let $[r]^+ \:= \text{max}(r, 0)$, and $\lfloor r \rfloor$ to be the largest integer no greater than $r$.



==> Convergence in a Repeated Non-atomic Routing Game with Partial Signaling/lit-review.tex <==
\section{Literature Review}








==> Convergence in a Repeated Non-atomic Routing Game with Partial Signaling/model.tex <==
\section{Model}
\label{sec:model}

\input{non-atomic}

%\input{correlated-equilibrium}

\input{dynamics}

==> Convergence in a Repeated Non-atomic Routing Game with Partial Signaling/non-atomic.tex <==
\subsection{Non-atomic Routing Game with Partial Signaling}

Consider a network consisting of $\nlinks$ parallel links between a single source-destination pair. Without loss of generality, let the agent population generate a unit volume of traffic demand. 
%Consider a network consisting of a directed acyclic graph from a single origin to a single destination. Let the paths from from the origin to the destination be indexed as $\{1, \ldots, \npaths\}$, and let the directed links be indexed as $\{1, \ldots, \nlinks\}$. Let $P \in \{0,1\}^{\npaths \times \nlinks}$ be the path-link matrix, where $P_{i,j}=1$ if and only if link $j$ belongs to path $i$. A unit volume, without loss of generality, of traffic demand needs to be routed from the origin to the destination. 
The link latency functions $\congfunc_{\omega,i}(f_i)$, $i \in [\nlinks]$, give latency on link $i$ as a function of flow $f_i$ through them, conditional on the \emph{state} of the network $\state \in \allstates=\{\state_1, \ldots,\state_{\nstates}\}$. Throughout the paper, we shall make the following basic assumption on these functions.
\begin{assumption}
\label{ass:continuous}
For every $i \in [\nlinks]$, $\state \in \Omega$, $\congfunc_{\omega,i}$ is a non-negative, continuously differentiable and non-decreasing function.
\end{assumption}
At times, we shall strengthen the assumption to $\congfunc_{\omega,i}$ being strictly increasing. For Proposition~\ref{prop:homo}, Lemma~\ref{lemma:convergence}, Lemma~\ref{lemma:lipschitz} and Theorem~\ref{prop:convergence}, we restrict ourselves to general polynomial latency function in the following form:
\begin{equation}
\label{eq:polynomial-latency-function}
\congfunc_{\omega,i}(f_i) =  \sum^D_{d=0} \alpha_{d,\omega,i} \, f_i^d, \, i \in [\nlinks], \, \, \state \in \allstates
\end{equation}
with $\alpha_{0,\state,i} \geq 0$ and $\alpha_{1,\state,i} \geq 0$. We shall also let $\alpha_{d,\omega}$ refer to the $\nlinks \times 1$ column vector whose entries are $\alpha_{d,\state,i}$, and $\alpha_d$ refer to the $\nstates \times \nlinks$ matrix whose entries are $\alpha_{d,\state,i}$.

Let $\state \sim \prior \in \interior(\triangle(\allstates))$, for some prior $\prior$ which is known to all the agents. 
%We assume that the average value of the linear coefficient in \eqref{eq:latency-affine} is strictly positive, i.e.,  Let $\overline{\beta}_i:=\sum_{\state} \prior(\state) \beta_i^{\state}$ denote the average value of the affine term in \eqref{eq:latency-affine}.  
The agents do not have access to the realization of $\state$, but a fixed fraction $\pfrac \in [0,1]$ of the agents receives private route recommendations conditional on the realized state. These conditional recommendations are generated by a \emph{signal} $\signal=\{\signal_{\state} \in \simplex_{\nlinks}(\pfrac): \, \state \in \allstates\}$.

\begin{remark}
The signal defined above is \emph{diagonal atomic}~\cite{Zhu.Savla:TCNS20}. A generalization is $\signal=\{\signal_{\state} \in \triangle(\simplex_{\nlinks}(\pfrac)): \, \state \in \allstates\}$. We postpone consideration of such a general setting to future work. 
\end{remark}

==> Convergence in a Repeated Non-atomic Routing Game with Partial Signaling/notations.tex <==
\section{Notations}
Let $(n):=\{1,\ldots,n\}$ be the set of integers from 1 thru $n$.

==> Convergence in a Repeated Non-atomic Routing Game with Partial Signaling/proofs.tex <==
\subsection{Proof of Proposition~\ref{prop:homo}}
Plugging \eqref{eq:instant} into \eqref{eq:S-agent-update} and substituting \eqref{eq:p flow dynamics-m-general-matrix} gives
\begin{align}
%\begin{aligned}
m(k) = & \frac{m(1)}{k}+\frac{1}{k} \sum_{t=1}^{k-1} u(t) \nonumber \\
=&\frac{m(1)}{k}+\frac{1}{k} \sum_{t=1}^{k-1} {\pi_{\omega(t)}}^T (I-P) \congfunc_{\omega(t)}(x(t)) \nonumber \\
=&\frac{m(1)}{k}+\frac{1}{k} \sum_{t=1}^{k-1} {\pi_{\omega(t)}}^T (I-P) \left(\alpha_{0,\omega(t)} + \sum_{d=1}^D \diag(\alpha_{d,\omega(t)}) \diag(x(t))^{d-1} x(t)\right) \nonumber \\
\label{eq:mistrust-m1-general}
= & \frac{m(1)}{k}+\frac{1}{k} \sum_{t=1}^{k-1} {\pi_{\omega(t)}}^T (I-P) \left(\ell_{\omega(t)}(\pi_{\omega(t)}) + \sum_{d=1}^D \diag(\alpha_{d,\omega(t)}) \left(\diag(x(t))^{d-1} x(t) - \diag(\pi_{\omega(t)})^{d-1} \pi_{\omega(t)}\right) \right) \nonumber \\
= & \frac{m(1)}{k}+\frac{1}{k} \sum_{t=1}^{k-1} {\pi_{\omega(t)}}^T (I-P) \ell_{\omega(t)}(\pi_{\omega(t)}) \nonumber \\
& \qquad \qquad \quad - \frac{1}{k} \sum_{t=1}^{k-1} \theta(t) \underbrace{{\pi_{\omega(t)}}^T (I-P) \sum_{d=1}^D \diag(\alpha_{d,\omega(t)}) \sum_{i=0}^{d-1} \diag(x(t))^{d-1-i} \diag(\pi_{\omega(t)})^{i}  (I-P^T) \pi_{\omega(t)}}_{\geq 0} \nonumber \\
\leq &  \frac{m(1)}{k}+\frac{1}{k} \sum_{t=1}^{k-1} {\pi_{\omega(t)}}^T (I-P) \congfunc_{\omega(t)}(\pi_{\omega(t)}) \nonumber \\
= &  \frac{m(1)}{k}+\sum_{i, j \in [n]} P_{ij} \frac{1}{k} \sum_{t=1}^{k-1} \pi_{\omega(t),i} \left(\congfunc_{\omega(t),i}(\pi_{\omega(t)})-\congfunc_{\omega(t),j}(\pi_{\omega(t)})\right)
\end{align}
\eqref{eq:obedience-hetero-v1} and the strong law of large numbers implies that, almost surely, 
$\lim_{k \to \infty}\frac{1}{k} \sum_{t=1}^{k-1} \pi_{\omega(t),i} \\ \left(\congfunc_{\omega(t),i}(\pi_{\omega(t)}) -\congfunc_{\omega(t),j}(\pi_{\omega(t)})\right) \leq 0$ for all $i, j \in [n]$, and therefore, almost surely, $\limsup_{k \to \infty} m(k) \leq 0$, and hence $\lim_{k \to \infty} \theta(k)=0$ from \eqref{eq:rating-to-mistrust}. The proposition then follows from \eqref{eq:p flow dynamics-m-general-matrix}. 

\subsection{Proof of Proposition~\ref{prop:convergence-lambda-zero}}
\eqref{eq:smoothing-model} implies $e_{\theta}(k+1) = (1-\beta(k+1)) e_{\theta}(k)$, and hence $e_{\theta}(k+1)=\prod_{t=2}^{k+1} (1-\beta(t)) e_{\theta}(1)$. The proposition then follows from the fact that $(1-\beta_{\max})^k e_{\theta}(1) \leq e_{\theta}(k+1) \leq (1-\beta_{\min})^k e_{\theta}(1)$.

\subsection{Proof of Proposition~\ref{prop:gamma-lambda-non-zero}}
\eqref{eq:smoothing-model} implies
\begin{equation}
\label{eq:P-dynamic}
\begin{aligned}
e_{\theta}(k+1) = (1- \beta(k+1)) e_{\theta}(k)+\delta(k)
%\frac{[M(k)]^+-[M(k+1)]^+}{\mu_M}
\end{aligned}
\end{equation}
where %$c_{k+1}$ is described by \eqref{eq:c}, 
$\delta(k)=\theta(k+1)-\theta(k)$. Using the expression of $\theta$ from \eqref{eq:rating-to-mistrust} and noting that $\left|[a]^+-[b]^+\right|\leq[a-b]^+$ for all $a, b \in \mathbb{R}$, we get
\begin{align*}
\frac{-[u(k)-m(k)]^+}{(k+1) m_{\max}} &\leq \delta(k) \leq \frac{[u(k)-m(k)]^+}{(k+1) m_{\max}}
\end{align*}
Since $[a-b]^+\leq|a|+|b|$ for all $a, b \in \mathbb{R}$, and both $m(k)$ and $u(k)$ are absolutely upper bounded by $m_{\max}$,  %$\frac{-2}{k+1} \leq \Delta_{k} \leq \frac{2}{k+1}$, which implies that for any $\epsilon>0, \exists K>0, s.t. |\Delta_k|\leq \epsilon, \forall k\geq K$. Thus, for any $\epsilon>0, \exists K>0, s.t. \forall k\geq K, |x_{k}| \leq |x_{k-1}|+\epsilon, \text{among which } |x_{k}| \leq (1-c_{min})|x_{k-1}|+\epsilon$ occurs infinitely often as $k \to \infty$ almost surely. Therefore, we can establish that, almost surely, $\lim_{k \to \infty} x_k=0$.
\begin{equation}
\label{eq:harmonic-bound}
\frac{-2}{k+1} \leq \delta(k) \leq \frac{2}{k+1}
\end{equation}
Since $\delta(k)$ can only be bounded by a harmonic sequence whose partial sum sequence diverges, it is not easy to prove that $\lim_{k \to \infty} e_{\theta}(k)=0$ directly using \eqref{eq:P-dynamic}. Instead, we lower and upper bound $e(k)$ by $\underline{e}_{\theta}(k)$ and $\overline{e}_{\theta}(k)$, respectively, and show that these converge to zero. \eqref{eq:P-dynamic} can be rewritten as
\begin{equation}
\label{eq:e-explicit}
e_{\theta}(k)=\left(\prod_{t=2}^{k} (1- \beta(t))\right) e_{\theta}(1)+ \sum_{t=1}^{k-2} \left(\prod_{\tau=t+2}^{k} (1- \beta(\tau))\right) \delta(t) + \delta(k-1)
\end{equation}
Substituting \eqref{eq:harmonic-bound} into \eqref{eq:e-explicit},
\begin{equation}
\label{eq:e-bound}
\underline{e}_{\theta}(k) := \left(\prod_{t=2}^{k} (1- \beta(t))\right) e_{\theta}(1)-2 \tilde{\delta}(k) \leq e_{\theta}(k) \leq \left(\prod_{t=2}^{k} (1- \beta(t))\right) e_{\theta}(1)+2 \tilde{\delta}(k)=:\overline{e}_{\theta}(k)
\end{equation}
where $\tilde{\delta}(k)=\sum_{t=2}^{k} (1- \beta_{\min})^{k-t} \frac{1}{t}= \gamma^{k}\sum_{t=2}^{k} \frac{\gamma^{-t}}{t}$, with $\gamma:=1-\beta_{\min} \in (0,1)$. $\frac{\gamma^{-t}}{t}$ is decreasing over $(0,-\frac{1}{\ln \gamma}]$, and increasing over $[-\frac{1}{\ln \gamma},+\infty)$. Therefore, with $k^*:=\lfloor -\frac{1}{\ln \gamma}\rfloor$,
\begin{equation*}
\begin{split}
\tilde{\delta}(k) & = \gamma^k \left(\sum_{t=2}^{k^*} \frac{\gamma^{-t}}{t} + \sum_{t=k^*+1}^k \frac{\gamma^{-t}}{t}\right) \leq \gamma^k \left( \int_1^{k^*} \frac{\gamma^{-t}}{t}  \de t + \int_{k^*+1}^{k+1} \frac{\gamma^{-t}}{t}  \de t\right) \leq \gamma^k \underbrace{\int_1^{k+1} \frac{\gamma^{-t}}{t}  \de t}_{=:I_{k+1}}
\end{split}
\end{equation*}
\ksmarginphantom{need a reference}
Change of variable $z=\gamma^{-t}$ gives
%\begin{equation*}
$I_{k+1} = \int_{\gamma^{-1}}^{\gamma^{-(k+1)}} \frac{\de z}{\ln z}=\mathrm{Li}(\gamma^{-(k+1)})-\mathrm{Li}(\gamma^{-1})$, where $\mathrm{Li}(\cdot)$ is the logarithmic integral function \cite{abramowitz1964} whose asymptotic behavior is $\mathrm{Li}(r)=O(\frac{r}{\ln r})$. 
%\end{equation*}
%\kscomment{[old stuff ...]}
%
%To show that $\tilde{\delta}(k)$ converges to zero, let us consider the continuous approximation using $g(t)=\frac{\gamma^{-t}}{t}$, where $\gamma=1-\beta_{min}\in (0,1)$. Since for $\forall t>0$, $g(t)>0$, and $g'(t)=\gamma^{-t-1}\frac{-t^2-\gamma}{t^2}<0$, we have for $\forall t>0$, $g(t)\leq \int_t^{t+1} g(\tau) d\tau$, thus
%
%\begin{equation*}
%\tilde{\delta}(k)=\gamma^{k} \sum_{t=2}^{k} g(t) \leq \gamma^{k} \int_2^{k+1} g(\tau) d\tau=\gamma^k  \underbrace{\int_2^{k+1} \frac{\gamma^{-\tau}}{\tau}d\tau}_{I_k}
%\end{equation*}
% Consider the change of variable $z=\gamma^{-\tau}$, which leads to $\tau=-\frac{ln(z)}{ln(\gamma)}, d\tau=-\frac{dz}{ln(\gamma)z}$, substitute into $I_k$ we have
%\begin{equation*}
%I_k=\int_{\gamma^{-2}}^{\gamma^{-(k+1)}} z \left(-\frac{ln(\gamma)}{ln(z)}\right) \left(-\frac{dz}{ln(\gamma)z}\right)=\int_{\gamma^{-2}}^{\gamma^{-(k+1)}} \frac{dz}{ln(z)}=Li(\gamma^{-(k+1)})-Li(\gamma^{-2})
%\end{equation*}
%\ksmargin{need a reference}
%where $Li(\cdot)$ is the \kscomment{logarithmic integral function whose asymptotic behavior is $Li(s)=O(\frac{s}{ln(s)})$}. 
Since $\gamma \in (0,1)$, $\gamma^{-(k+1)} \to \infty$ as $k \to \infty$. Therefore, as $k \to \infty$,
\begin{equation*}
\begin{aligned}
0<\tilde{\delta}(k)\leq \gamma^k \left(\mathrm{Li}(\gamma^{-(k+1)})-\mathrm{Li}(\gamma^{-1})\right)&=\gamma^k \left(O\left(\frac{\gamma^{-(k+1)}}{-(k+1) \ln \gamma}\right)-\mathrm{Li}(\gamma^{-1})\right) \\
&=O\left(\frac{\gamma^{-1}}{-(k+1) \ln \gamma}\right)-\gamma^k \mathrm{Li}(\gamma^{-1}) \to 0
\end{aligned}
\end{equation*}
which leads to $\lim_{k \to \infty} \tilde{\delta}(k) =0$. Using it in \eqref{eq:e-bound} therefore gives $\lim_{k \to \infty}\underline{e}_{\theta}(k)=0$ and $\lim_{k \to \infty}\overline{e}_{\theta}(k)=0$, and hence $\lim_{k \to \infty} e_{\theta}(k)=0$.
%
%Comparing trends of functions $-\ln(1-\beta_{\min})(k-1)$ and $\ln(k+1)$, it is easy to see that $-\ln(1-\beta_{\min})(k-1)>\ln(k+1)$, i.e.,  $\frac{1}{k+1}-\frac{\big(1-(1-\beta_{\min})^{k-1}\big)}{k}<0$, for all sufficiently large $k$.
%% Since $g_1(0)<g_2(0)$, and for $k>-\frac{1}{ln(1-\beta_{\min})}-1$, $g_1(k)'>g_2(k)'>0$, there $\exists K>0$ s.t. $g_1(k)>g_2(k), \forall k>K$. That is, for $k>K$, we have $-ln(1-\beta_{\min})(k-1)>ln(k+1)$, which gives us $(k+1)(1-\beta_{\min})^{k-1}<1$, or equivalently $\frac{1}{k+1}-\frac{\big(1-(1-\beta_{\min})^{k-1}\big)}{k}<0$. %$g_1(k)$ is a affine function with positive slope $-lg(1-\beta_{\min})$ and negative intercept $lg(1-\beta_{\min})$. $g_2(k)$ is a logarithm function which increases slower than the affine function $g_1(k)$ with intercept equals zero. 
%Combining this with the fact that $\tilde{\delta}(k)>0$ for all $k$, 
%\begin{equation*}
%\label{eq:e-difference}
%\begin{aligned}
%\tilde{\delta}[k+1]-\tilde{\delta}(k)&= \frac{1}{k+1}-\beta_{\min} \tilde{\delta}(k) =\frac{1}{k+1}-\beta_{\min} \sum_{t=1}^{k-1} (1- \beta_{\min})^{k-t-1} \frac{1}{t+1} \\
%&<\frac{1}{k+1}-\beta_{\min} \sum_{t=1}^{k-1} (1- \beta_{\min})^{k-t-1} \frac{1}{k} =\frac{1}{k+1}-\frac{\big(1-(1-\beta_{\min})^{k-1}\big)}{k} \\
%&<0
%\end{aligned}
%\end{equation*}
%for all sufficiently large $k$.
%\kscomment{Therefore, using D'Alembert's test, we get $\lim_{k \to \infty} \tilde{\delta}(k) =0$.} Using this in \eqref{eq:e-bound} therefore gives $\lim_{k \to \infty}\underline{e}_{\theta}(k)=0$ and $\lim_{k \to \infty}\overline{e}_{\theta}(k)=0$, and hence $\lim_{k \to \infty} e_{\theta}(k)=0$.

\subsection{Proof of Lemma~\ref{lemma:convergence}}
Plugging \eqref{eq:instant} into \eqref{eq:S-agent-update} and substituting \eqref{eq:p flow dynamics-m-general-matrix} gives the following:
\begin{align}
m(k) = & \frac{m(1)}{k}+\frac{1}{k} \sum_{t=1}^{k-1} {\pi(t)}^T (I-P) \left(\alpha_{0,\omega(t)} + \sum_{d=1}^D \diag(\alpha_{d,\omega(t)}) \diag(x(t)+y(\hat{\theta}(t)))^{d-1} \left(x(t)+y(\hat{\theta}(t))\right)\right) \nonumber \\
\label{eq:m-split-general}
= & \frac{m(1)}{k}+\frac{1}{k} \sum_{t=1}^{k-1} {\pi(t)}^T (I-P) \left(\alpha_{0,\omega(t)} + \sum_{d=1}^D \diag(\alpha_{d,\omega(t)}) \diag(\nu \pi_{\omega(t)}+y(0))^{d-1} \left(\nu \pi_{\omega(t)}+y(0)\right)\right) \nonumber \\
& + \frac{1}{k} \sum_{t=1}^{k-1} {\pi(t)}^T (I-P) \sum_{d=1}^D \diag(\alpha_{d,\omega(t)}) \Bigg(\diag(x(t)+y(\hat{\theta}(t)))^{d-1} \left(x(t)+y(\hat{\theta}(t))\right) \nonumber \\
& \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad - \diag(\nu \pi_{\omega(t)}+y(0))^{d-1} \left(\nu \pi_{\omega(t)}+y(0)\right)\Bigg) \nonumber \\
= & \frac{m(1)}{k}+\frac{1}{k} \sum_{t=1}^{k-1} {\pi(t)}^T (I-P) \left(\alpha_{0,\omega(t)} + \sum_{d=1}^D \diag(\alpha_{d,\omega(t)}) \diag(\nu \pi_{\omega(t)}+y(0))^{d-1} \left(\nu \pi_{\omega(t)}+y(0)\right)\right) \nonumber \\
& + \frac{1}{k} \sum_{t=1}^{k-1} {\pi(t)}^T (I-P) \sum_{d=1}^D \diag(\alpha_{d,\omega(t)}) \sum_{i=0}^{d-1} \diag(x(t)+y(\hat{\theta}(t)))^{d-1-i} \diag(\nu \pi_{\omega(t)}+y(0))^{i} \cdot \nonumber \\
& \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \left(\nu \theta(t)(P^T-I) \pi_{\omega(t)}+y(\hat{\theta}(t))-y(0)\right)
\end{align}

Since $m(k)$ is a bounded sequence, it contains a convergent subsequence $\{m((k_s)\}_s$ with limit, say, $m$. Considering \eqref{eq:m-split-general} for this subsequence, using Proposition~\ref{prop:gamma-lambda-non-zero} we have, almost surely, 
\ksmarginphantom{need to check this step carefully}
\begin{align}
\label{eq:m-split-general-limit}
m = & \underbrace{\sum_{\omega \in \Omega} \prior(\omega) {\pi_{\omega}}^T (I-P) \left(\alpha_{0,\omega} + \sum_{d=1}^D \diag(\alpha_{d,\omega}) \diag(\nu \pi_{\omega}+y(0))^{d-1} \left(\nu \pi_{\omega}+y(0)\right)\right)}_{=:m_1} \nonumber \\
& + \underbrace{\sum_{\omega \in \Omega} \prior(\omega)  {\pi_{\omega}}^T (I-P) \sum_{d=1}^D \diag(\alpha_{d,\omega}) \sum_{i=0}^{d-1} \diag(x(m, \pi_{\omega})+y(\theta(m)))^{d-1-i} \diag(\nu \pi_{\omega}+y(0))^{i} \cdot}_{=:m_2} \nonumber \\
& \quad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \underbrace{\left(\nu \theta(m)(P^T-I) \pi_{\omega}+y(\theta(m))-y(0)\right)}_{=:m_2}
\end{align}
i.e., the limit $m$ of every convergent subsequence of $\{m(k)\}_k$ has to satisfy \eqref{eq:m-split-general-limit}. We now show that \eqref{eq:m-split-general-limit} admits a unique solution in $m$, and that this solution is non-positive. Towards that purpose, the following properties of $m_1$ and $m_2$ defined in \eqref{eq:m-split-general-limit} will be useful:
\begin{enumerate}
\item[(a)] $m_1 \leq 0$ for all $m$. This is due to the obedience condition;
\item[(b)] $m_2=0$ for all $m \leq 0$. This follows from the definition of $m_2$, where $\theta(m)=0$ for $m \leq 0$ from \eqref{eq:rating-to-mistrust};
\item[(c)] $m_2 \leq 0$ for all $m>0$, as follows. \eqref{eq:BEW-VI-matrix} for $y(\theta(m))$ and $y(0)$, respectively, give:
\end{enumerate} 
\begin{align}
&\sum_{\omega \in \Omega} \prior(\omega) (y(0)-y(\theta(m)))^T \Bigg(\alpha_{0,\omega} + \sum_{d=1}^D \diag(\alpha_{d,\omega}) \diag(x(m, \pi_{\omega})+y(\theta(m)))^{d-1} \left(x(m, \pi_{\omega})+y(\theta(m))\right)\Bigg) \geq 0 \nonumber \\
&\sum_{\omega \in \Omega} \prior(\omega) (y(\theta(m))-y(0))^T \Bigg(\alpha_{0,\omega} + \sum_{d=1}^D \diag(\alpha_{d,\omega}) \diag(\pfrac \signal_{\omega} + y(0))^{d-1} \left(\pfrac \signal_{\omega} + y(0)\right)\Bigg) \geq 0 \nonumber
\end{align}

Adding the two expressions gives
%\begin{equation*}
\begin{align}
\label{eq:expr-add}
&\sum_{\omega \in \Omega} \prior(\omega)  (y(0)-y(\theta(m)))^T \sum_{d=1}^D \diag(\alpha_{d,\omega}) \Bigg(\diag(x(m, \pi_{\omega})+y(\theta(m)))^{d-1} \left(x(m, \pi_{\omega})+y(\theta(m))\right) \nonumber \\
& - \diag(\pfrac \signal_{\omega} + y(0))^{d-1} \left(\pfrac \signal_{\omega} + y(0)\right)\Bigg) \nonumber \\
= & \sum_{\omega \in \Omega} \prior(\omega)  (y(0)-y(\theta(m)))^T \sum_{d=1}^D \diag(\alpha_{d,\omega}) \sum_{i=0}^{d-1} \diag(x(m, \pi_{\omega})+y(\theta(m)))^{d-1-i} \diag(\nu \pi_{\omega}+y(0))^{i} \cdot \nonumber \\
& \quad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \left(\nu \theta(m)(P^T-I) \pi_{\omega}+y(\theta(m))-y(0)\right) \geq 0
\end{align}

Finally, 
\begin{align}
m_2 =&  -\frac{1}{\pfrac \theta(m)} \underbrace{\sum_{\omega \in \Omega} \prior(\omega) \left(\pfrac \theta(m) {\pi_{\omega}}^T (P -I)  + y^T(\theta(m)) - y^T(0)\right)  \sum_{d=1}^D \diag(\alpha_{d,\omega}) \cdot}_{=:m_3 \geq 0} \nonumber \\
& \underbrace{\sum_{i=0}^{d-1} \diag(x(m, \pi_{\omega})+y(\theta(m)))^{d-1-i} \diag(\nu \pi_{\omega}+y(0))^{i} \left(\nu \theta(m)(P^T-I) \pi_{\omega}+y(\theta(m))-y(0)\right)}_{=:m_3 \geq 0} \nonumber\\
&-\frac{1}{\pfrac \theta(m)} \underbrace{\sum_{\omega \in \Omega} \prior(\omega)  (y(0)-y(\theta(m)))^T \sum_{d=1}^D \diag(\alpha_{d,\omega})  \cdot}_{=:m_4 \geq 0 \text{ from \eqref{eq:expr-add}}} \nonumber \\
& \underbrace{\sum_{i=0}^{d-1} \diag(x(m, \pi_{\omega})+y(\theta(m)))^{d-1-i} \diag(\nu \pi_{\omega}+y(0))^{i} \left(\pfrac \theta(m)  (P^T -I) \pi^{\omega} + y(\theta(m)) - y(0)\right)}_{=:m_4 \geq 0 \text{ from \eqref{eq:expr-add}}} \nonumber
\end{align}
where we note that $\theta(m)>0$ for $m>0$.

(a), (b) and (c) imply that the right hand side of \eqref{eq:m-split-general-limit} is always non-positive. (a) and (b) also imply that the only non-positive solution to \eqref{eq:m-split-general-limit} is $m = m_1$.

\subsection{Proof of Lemma~\ref{lemma:lipschitz}}
Along the lines of Theorem 1 in \cite{Dempe1997}, we just need to verify the following three conditions: Mangasarian-Fromowitz constraint qualification (MF), strong sufficient optimality condition of second order (SOC), and constant rank constraint qualification (CR). Plugging in \eqref{eq:polynomial-latency-function} and rewriting the latency function in \eqref{eq:BWE} gives:
\begin{align}
\label{eq:BWE-latency}
\ell_{\omega,i}(\hat{x}_i(\theta,\omega)+y_i) = \sum_{d=0}^D \alpha_{d,\omega,i} (\nu \pi_{\omega.i} + \nu \theta P_i^T \pi_{\omega} - \nu \theta \pi_{\omega,i} + y_i) = \alpha_{D,\omega,i} y_i^D + \sum_{d=0}^{D-1} \beta_{d,\omega,i} y_i^d
\end{align}
where $P_i \in \real^n$ is the $i$-th column of the row-stochastic matrix $P$, and $\beta_{d,\omega,i}(\{\alpha_{k,\omega,i}\}_{k \in \{0,1,\cdots,D\}}, \pi_{\omega},\theta,P_i)$ is the coefficient of monomial of degree $d$. Taking expectation of \eqref{eq:BWE-latency} gives:
 \begin{align}
E_{\omega \sim \prior} [\ell_{\omega,i}(\hat{x}_i(\theta,\omega)+y_i)] = E_{\omega \sim \prior} [\alpha_{D,\omega,i} y_i^D + \sum_{d=0}^{D-1} \beta_{d,\omega,i} y_i^d]=\bar{\alpha}_{D,i}y_i^D + \sum_{d=0}^{D-1} \bar{\beta}_{d,i} y_i^d \nonumber
\end{align}
where $\bar{\alpha}_{D,i}:=E_{\omega \sim \prior} [\alpha_{D,\omega,i}], \bar{\beta}_{d,i}:=E_{\omega \sim \prior} [\beta_{d,\omega,i}]$. $y(\theta)$ satisfies \eqref{eq:BWE} if and only if it solves the following convex problem:
\begin{equation}
\label{prob:BWE}
\begin{aligned}
\min_{y \in \simplex_n(1-\nu)} &f(y,\theta)=\sum_{i \in [n]} \int_0^{y_i} E_{\omega \sim \prior} [\ell_{\omega,i}(\hat{x}_i(\theta,\omega)+s)] ds = \sum_{i \in [n]} \left(\frac{\bar{\alpha}_{D,i}}{D+1}y_i^{D+1} + \sum_{d=0}^{D-1} \frac{\bar{\beta}_{d,i}}{d+1} y_i^{d+1}\right) \\
\text{s.t.} \quad &g_i(y,\theta) = -y_i \leq 0, \, i \in [n] \\
&h(y,\theta)=\sum_{i=1}^n y_i -1+\nu
\end{aligned}
\end{equation}
Moreover, such $y$ is unique if $\{\ell_{\omega,i}\}_{\omega,i}$ are strictly increasing over $[0,1]$. Let the Lagrange function be $L(y,\theta,\lambda, \mu)=f(y,\theta)-\sum_{i \in [n]} \lambda_i y_i + \mu(\sum_{i=1}^n y_i -1+\nu)$. For a given $\theta^0$, $y=y^0$ is a locally optimal solution for \eqref{prob:BWE} at $\theta=\theta^0$. Now, we want to show that $y(\theta)$ is Lipschitz continuous by verifying aforementioned three conditions. 

(MF) From \eqref{prob:BWE} we have:
\begin{align}
\nabla_y g_i(y^0, \theta^0) = \begin{bmatrix}0\\ \vdots \\ -1\\ \vdots \\0\end{bmatrix}_{n \times 1}\leftarrow \text{i-th entry} \qquad \nabla_y h(y^0, \theta^0) = \begin{bmatrix}1\\1\\ \vdots \\ 1\end{bmatrix}_{n \times 1} \nonumber
\end{align}
Obviously, $\nabla_y h(y^0, \theta^0)$ is linearly independent. Let $v \in \real^n$ be such that:
\begin{equation*}
v_i=
\begin{cases}
1&\text{if} \, \, g_i(y^0, \theta^0)=0 \\
\frac{\sum_{i \in [n]}\mathbbm{1}(g_i(y^0, \theta^0)=0)}{\sum_{i \in [n]}\mathbbm{1}(g_i(y^0, \theta^0)=0)-n}&\text{if} \, \, g_i(y^0, \theta^0)\neq 0
\end{cases}
\end{equation*}
$v$ satisfies that:
\begin{align}
&\nabla_y g_i(y^0, \theta^0)^T v < 0, \quad \text{for} \, \, g_i(y^0, \theta^0)=0 \nonumber \\
&\nabla_y h(y^0, \theta^0)^T v = 0 \nonumber
\end{align}

(SOC) Let $\{H_{ij}\}_{i,j \in [n]}:=\nabla^2_{yy} L(y^0,\theta^0,\lambda, \mu)$, from \eqref{prob:BWE} we have:
\begin{equation*}
H_{ij}=
\begin{cases}
0&\text{if} \, \, i \neq j \\
D \bar{\alpha}_{D,i} y_i^{D-1}+\sum_{d=1}^{D-1} d \bar{\beta}_{d,i} y_i^{d-1}&\text{if} \, \, i=j
\end{cases}
\end{equation*}
which implies that for $\forall v \in \real^n, \, v \neq0$, we have $v^T \nabla^2_{yy} L(y^0,\theta^0,\lambda, \mu) v > 0$.

(CR) Let $I_0:=\{i | g_i(y^0, \theta^0) = 0\}$, $I$ is arbitrary but fixed subset $I \subseteq I_0$. Note that, $\sum_{i \in [n]} \mathbbm{1}(g_i(y^0, \theta^0)=0) \leq n-1$, therefore the set of gradients $\{\nabla_y g_i(y^0, \theta^0), \, i \in I\} \cup \{\nabla_y h(y^0, \theta^0)\}$ has constant rank $|I|+1$, for all $(y,\theta)$ in open neighborhood of $(y^0,\theta^0)$.

\subsection{Proof of Theorem~\ref{prop:convergence}}
Following \eqref{eq:p flow dynamics-m-general-matrix}, it suffices to show that $\lim_{k \to \infty} \theta(m(k))=0$, almost surely.

Lemma~\ref{lemma:convergence} shows that there exists a convergent subsequence $\{m(k_s)\}_s$ with limit $m \leq 0$, almost surely. That is, there exists $\tilde{s}_1>0$ such that 
\begin{equation}
\label{eq:eps1}
|m(k_s)-m|\leq -m/3 \quad \forall  s>\tilde{s}_1 \quad \text{a.s.}
\end{equation}

We now show that all the terms of the parent sequence $m(k)$ between two consecutive subsequence terms $m(k_s)$ and $m(k_{s+1})$, for $s>\tilde{s}_1$, are negative.
\eqref{eq:S-agent-update} implies, for all $s > \tilde{s}_1$,  
\begin{equation*}
m(k_s+1) = \frac{k_s}{k_s+1} m(k_s) + \frac{1}{k_s+1} u_0(k_s) + \frac{1}{k_s+1} \triangle u(k_s) 
\end{equation*}
i.e., 
\begin{equation}
\label{eq:trust-update-subsequence-delta}
m(k_s+1) - m = \frac{k_s}{k_s+1} \left(m(k_s) -m \right)+ \frac{1}{k_s+1} \left(u_0(k_s) - m \right)+ \frac{1}{k_s+1} \triangle u(k_s) 
\end{equation}
where 
\begin{equation*}
u_0(k_s):={\pi_{\omega(k_s)}}^T (I-P) \left(\alpha_{0,\omega(k_s)} + \sum_{d=1}^D \diag(\alpha_{d,\omega(k_s)}) \diag(\pfrac \signal_{\omega(k_s)} + y(0))^{d-1} \left(\pfrac \signal_{\omega(k_s)} + y(0)\right)\right)
\end{equation*}
be the instantaneous mistrust assuming B-agents estimate that P-agents are obedient, i.e., assuming $\hat{\theta}(k_s)=0$, and 
\begin{align}
& \triangle u(k_s) :=  u(k_s) - u_0(k_s) \nonumber \\
 = & {\pi_{\omega(k_s)}}^T (I-P) \sum_{d=1}^D \diag(\alpha_{d,\omega(k_s)}) \Bigg(\diag(x(k_s)+y(\hat{\theta}(k_s)))^{d-1} \left(x(k_s)+y(\hat{\theta}(k_s))\right) \nonumber \\
 & - \diag(\pfrac \signal_{\omega(k_s)} + y(0))^{d-1} \left(\pfrac \signal_{\omega(k_s)} + y(0)\right)\Bigg) \nonumber \\
 = & {\pi_{\omega(k_s)}}^T (I-P) \sum_{d=1}^D \diag(\alpha_{d,\omega(k_s)}) \sum_{i=0}^{d-1} \diag(x(k_s)+y(\hat{\theta}(k_s)))^{d-1-i} \diag(\nu \pi_{\omega(k_s)}+y(0))^{i} \left(y(\hat{\theta}(k_s))-y(0)\right)
\label{eq:delta-u}
\end{align}
In the above equations, we utilize \eqref{eq:eps1} to get $m(k_s)\leq 0$, and hence $\theta(m(k_s))=0$, for $s > \tilde{s}_1$. Using the Lipschitz property of $y(.)$ (cf. Remark~\ref{rem:BWE-lipschitz}) with \eqref{eq:delta-u} gives
\begin{equation}
\label{eq:delta-u-lipschitz}
|\triangle u(k_s)| \leq L |\hat{\theta}(k_s)|, \qquad s > \tilde{s}_1
\end{equation}
for some $L>0$. Proposition~\ref{prop:gamma-lambda-non-zero} implies that there exists $\tilde{k}_1>0$ such that $|\theta(m(k))-\hat{\theta}(k)| \leq - \frac{m}{3L}$ for all $k > \tilde{k}_1$. Let $\tilde{s}_2$ be the smallest integer greater than $\tilde{s}_1$ such that $k_{\tilde{s}_2}>\tilde{k}_1$. Therefore, $|\theta(m(k_s))-\hat{\theta}(k_s)|=|\hat{\theta}(k_s)| \leq - \frac{m}{3L}$ for all $s > \tilde{s}_2$. Combining with \eqref{eq:delta-u-lipschitz} gives
\begin{equation}
\label{eq:eps2}
|\triangle u(k_s)| \leq - \frac{m}{3}, \qquad s > \tilde{s}_2
\end{equation}

Strong law of large numbers gives $\lim_{\tau \to \infty}\left(\frac{\sum_{t=1}^{\tau}u_0(t)}{\tau}\right)=m$ almost surely, i.e., there exists $\tilde{k}_2$ such that $\left|\frac{\sum_{t=1}^{\tau} u_0(t)}{\tau} - m\right| \leq -m/6$ for all $\tau > \tilde{k}_2$. 
%Let $\tilde{s}_3$ be the smallest integer greater than $\tilde{s}_2$ such that $k_{\tilde{s}_3}>\tilde{k}_2$. 
Therefore, for all $\tau > \tilde{k}_2$ and a non-negative integer $r$,
\begin{equation*}
\begin{split}
\tau \frac{7m}{6} \leq  \sum_{t=1}^{\tau} u_0(t) \leq \tau \frac{5m}{6}, \qquad 
(\tau+1+r) \frac{7m}{6} \leq & \sum_{t=1}^{\tau+1+r} u_0(t) \leq (\tau+1+r) \frac{5m}{6}
%k \frac{7m}{6} \leq  m(1) + \sum_{t=1}^{k-1} u_0(t) \leq k \frac{5m}{6}, \qquad 
%(k+1) \frac{7m}{6} \leq & m(1) + \sum_{t=1}^{k} u_0(t) \leq (k+1) \frac{5m}{6}
\end{split}
\end{equation*}
Subtraction gives
\begin{equation}
\label{eq:eps3}
|\sum_{t=\tau+1}^{\tau+1+r}(u_0(t)-m)| \leq -(2\tau+r+1) \frac{m}{6}, \qquad  \tau > \tilde{k}_2,  r \geq 0
%\frac{m}{6} - 2 k  \leq u_0(k) - m \leq -\frac{m}{6} + 2 k, \qquad  k > \tilde{k}_2
\end{equation} 

Let $\tilde{s}$ be the smallest integer greater than $\tilde{s}_2$ such that $k_{\tilde{s}}>\tilde{k}_2$. Using \eqref{eq:eps1}, \eqref{eq:eps2} and \eqref{eq:eps3} ($\tau=k_s-1$, $r=0$) in \eqref{eq:trust-update-subsequence-delta} gives, for all $s > \tilde{s}$,
\begin{equation*}
|m(k_s+1)-m| \leq - \frac{k_s}{k_s+1} \frac{m}{3} - \frac{(2 k_s-1)}{k_s+1} \frac{m}{6}- \frac{1}{k_s+1}\frac{m}{3} < - \frac{2m}{3}
\end{equation*}
which implies that $m(k_s+1) < \frac{m}{3} \leq 0$. 

Hereafter, we show that $m(k_s+2), m(k_s+3), \ldots m(k_{s+1}-1)$ are all negative, for $s > \tilde{s}$, using induction. Let $m(t)<0$ for all $t \in \{k_s+1,\ldots,k-1\}$, for some $k \in \{k_s+2,\ldots,k_{s+1}-1\}$. Repeated application of \eqref{eq:trust-update-subsequence-delta} gives
\begin{equation}
\label{eq:trust-update-subsequence-delta-general}
m(k) -m = \frac{k_s}{k} (m(k_s)-m) + \frac{1}{k} \sum_{t=k_s}^{k-1} (u_0(t)-m) + \frac{1}{k} \sum_{t=k_s}^{k-1} \triangle u(t)
\end{equation}
Along similar lines as \eqref{eq:delta-u-lipschitz}, one can show that
%\begin{equation*}
$|\triangle u(t)| \leq - \frac{m}{3}$ for all $t \in \{k_s, \ldots, k-1\}$. 
%\end{equation*}
Using this, along with \eqref{eq:eps1} and \eqref{eq:eps3} ($\tau=k_s-1$, $r=k-k_s-1$), in \eqref{eq:trust-update-subsequence-delta-general} gives
\begin{equation*}
|m(k) -m| \leq - \frac{k_s}{k}\frac{m}{3} - \frac{(k+k_s-2)}{k}\frac{m}{6} - \frac{(k-k_s)}{k}\frac{m}{3} < - \frac{2m}{3}
\end{equation*} 
which implies that $m(k) < \frac{m}{3} \leq 0$. 
%\begin{equation}
%\label{eq:trust-update-subsequence}
%m(k_s+1) = \frac{k_s}{k_s+1} m(k_s) + \frac{1}{k_s+1} u(k_s)
%\end{equation}
%where $m-\epsilon_1 \leq m(k_s) \leq m+\epsilon_1 < 0$ for $s>\tilde{s}_1$. 
 

%Recall from \eqref{eq:instant} and \eqref{eq:p flow dynamics-m-general-matrix} that 
%\begin{equation*}
%u(k)={\pi(k)}^T (I-P) \left(\diag(\alpha_0(k)) + \diag(\alpha_1(k)) \left(\pfrac \pi^{\omega(k)} + \pfrac \theta(m(k)) (P^T - I ) \pi^{\omega(k)} + y(\hat{\theta}(k))\right)\right)
%\end{equation*}







==> Convergence in a Repeated Non-atomic Routing Game with Partial Signaling/regret-dynamics.tex <==
\subsection{Connection to Regret-Matching}
\label{sec:regret}
\cite{Hart.Mas-Colell:00} considers the following repeated game between finite players. In round $k$, a player who chose action $i$ in round $k-1$, switches to $j \neq i$ with probability $\frac{[m_{i \to j}(k)]^+}{m_{\max}}$, and sticks to $i$ with probability $1-\sum_{j\neq i}\frac{[m_{i \to j}(k)]^+}{m_{\max}}$, where $m_{i \to j}(k)$ is a measure of \emph{regret} for not having played $j$ every time that $i$ was played in the past, and the \emph{inertia} parameter $m_{\max}$ is sufficiently large to ensure that the probabilities are well defined. Formally, the regret is computed as: $m_{i \to j}(k):=\frac{1}{k-1}\sum_{t=1: \, \text{player chooses }i}^{k-1} (U(j, s^{-}(t))-U(s(t)))$, where $U$ is the utility function of the player under consideration, $s(t)$ is the set of actions chosen by all the players in round $t$, and $s^{-}(t)$ is the set of actions of all the players except the one under consideration. 

%the adaptive procedure that they propose guarantees convergence to the set of correlated equilibria of the game. Under such "regret-matching" procedure, assuming player $n$ chose strategy $i$ at time $k$, the conditional probability that the player switch to strategy $j \neq i$ at time $k+1$ is $\frac{[D_k^n(i,j)]^+}{\mu}$, where $D_k^n(i,j):=\frac{1}{k}\sum_{t=1: s_t^n=i}^k (u^n(j, s_t^{-n})-u^n(s_t))$ is a measure of the time-averaged "regret" for player $n$ at period $k$ for not having played strategy $j$ every time that $i$ was played in the past, and $\mu$ is a normalization factor that guarantees the probability that player $n$ sticks to strategy $i$ is positive, i.e. $1-\sum_{j\neq i}[\frac{D_k^n(i,j)]^+}{\mu}>0$. Here $s_t^n$ and $u_t^n$ are strategy and utility of player $n$ at time $t$ respectively.

\ksmarginphantom{does swapping the time average and population average sequence lead to the same model?}
%\ksmargin{YZ to check this}
The similarities and differences with the decision model of the $P$ agents in our setup is now apparent. An individual $P$ agent computes regret for its action to follow or to not to follow the recommendation in the previous round in the same spirit as \cite{Hart.Mas-Colell:00}. However, this regret is not categorized in terms of the specific action taken in the previous round. Such an absence of conditioning facilitates efficient aggregation of regrets of all the $P$ agents as a simple summation. The time-averaging of regrets is achieved through \eqref{eq:S-agent-update}, where $m_{\max}$ plays the role as the inertia parameter similar to \cite{Hart.Mas-Colell:00}.
%In our non-atomic setting, we again think of $P$-agents as a player. In light of the additional sender that \cite{Hart.Mas-Colell:00} does not consider, one can think of that the action space is changed from $n$-parallel links to following or not following the recommendations. Moreover, since we take perspective of all $P$-agents, an additional average over different strategies that different $P$-agents chose is taken in \eqref{eq:instant}. Thus \eqref{eq:S-agent-update} gives a measure of "regret" that is averaged not only over time but also over the entire population of $P$-agents. Our distinctive time- and population-averaged "regret" is hence no longer a conditional probability. Apart from the additional population-average that caused by our non-atomic setting, the method we construct "regret" in \eqref{eq:instant}, \eqref{eq:S-agent-update} and \eqref{eq:rating-to-mistrust}, and the way "regret" affects player's action in \eqref{eq:p flow dynamics-m-general-matrix} is not much different from \cite{Hart.Mas-Colell:00}.

==> Convergence in a Repeated Non-atomic Routing Game with Partial Signaling/simulation.tex <==
\section{Simulations}
\label{sec:simulation}
We report simulation results which suggest that the main convergence result is robust to natural variations of the dynamics in  \eqref{eq:instant}-\eqref{eq:smoothing-model}. We consider a network with two parallel links. 
Unless noted otherwise, in all the scenarios, 
%
%We conduct simulation of dynamics of both $\theta[k]$ and $\hat{\theta}[k]$ in three different scenarios. For all of the three scenarios, we show simulation results for the following choice of parameters: 
$\mu_0(\omega_1)=0.6=1-\mu_0(\omega_2)$, $\nu=0.5$, $\theta(1)=0.5$, $\hat{\theta}(1)=0.25$, and the total demand is set to be $1$. Also, the link latency functions are affine with coefficients: 
\begin{equation*}
\alpha_0 = 
\kbordermatrix{&i=1&i=2\\
\omega_1&5&25\\
\omega_2&20&15}, \quad 
\alpha_1 = 
\kbordermatrix{&i=1&i=2\\
\omega_1&4&2\\
\omega_2&1&2}
\end{equation*} 

%\ksmargin{YZ to update the plots}
\begin{figure}[htb!]
\begin{center}
\begin{minipage}[c]{.45\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{mistrust_convex_combination}
\\
(a)
\end{center}
\end{minipage}
\begin{minipage}[c]{.45\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{mistrust_varying_nu}
\\
(b)
\end{center}
\end{minipage}
\end{center}
\caption{\small \sf Convergence of regret and its forecast over two parallel links for (a) review aggregation with discounting factor $\lambda=0.9$, and (b) dynamic participation rate.}
\label{fig:simulation}
\end{figure}

In Scenario (a), we replace \eqref{eq:S-agent-update} with discounted review aggregation: $m(k+1)=\lambda m(k)+(1-\lambda)u(k)$. In Scenario (b), we let the participation rate also be dynamic, and in particular, we let $\nu(k)=\theta(k)$. Figure~\ref{fig:simulation}, which shows results for these scenarios, suggests that convergence of regret forecast as well as actual regret to zero is achieved even under these variations. 
%
%In Fig~\ref{fig:simulation}(b), instead of \eqref{eq:S-agent-update}, we use the following method to update $m[k]$: $m[k]=\lambda m[k-1]+(1-\lambda)u[k]$, where we choose $\lambda=0.9$. In Fig~\ref{fig:simulation}(c), we let $\nu[k]=\theta[k-1]$ to be time varying. In all of the three scenarios, we observe convergence of both regret forecast to actual regret and actual regret to zero.

==> estimation-models.tex <==
\subsection{Estimation Models for B-agents}
\label{sec:estimation}
We consider two classes of models for B-agents, inspired by Luenberger observer and exponential smoothing forecasting. 

\subsection{Luenberger-like estimation model}
In \eqref{eq:S-agent-update}-\eqref{eq:p flow dynamics-m-general}, one can interpret $m[k]$ as the state and $u[k]$ as the input driven by the output consisting of link latencies $\ell[k]=\{\ell_i^{\omega[k]}(x_i[k]+y_i[k]): \, i \in (n)\}$. The corresponding Luenberger-like observer therefore is:
\begin{equation}
\label{eq:luenberger-dynamics}
\hat{m}[k+1]=\frac{k}{k+1} \hat{m}[k] + \frac{1}{k+1} u[k] + L \left(\ell[k] - \hat{\ell}[k] \right)
\end{equation}
where $L$ is observer gain, and $\hat{\ell}[k]=\ell^{\omega[k]}\left(\hat{x}[k]+y[k]\right)$ is the estimated output. The estimation error is $e_m[k]:=m[k]-\hat{m}[k]$. The error dynamics is therefore
\begin{equation}
\label{eq:error-dynamics-luenberger}
e_m[k+1]=\frac{k}{k+1} e_m[k]- L \big(\ell[k]-\hat{\ell}[k]\big)
\end{equation}

\begin{proposition}
For every $m[1]$ and $\hat{m}[1]$, under \eqref{eq:error-dynamics-luenberger} with $L=0$, $\lim_{k \to \infty} e_m[k]=0$.
\end{proposition}
\begin{proof}
\eqref{eq:S-agent-update} can be rewritten as $m[k+1]=\frac{m[1]+\sum_{t=1}^k u[t]}{k+1}$. Using similar rewriting of \eqref{eq:luenberger-dynamics}, we get $e_m[k]=\frac{e_m[1]}{k}$, establishing the proposition.

\end{proof}

\subsection{Exponential smoothing estimation model}
Estimates produced using exponential smoothing methods are weighted averages of past observations, with the weights decaying exponentially as the observations get older. The \emph{simple} exponential smoothing model for the B-agent can be written in the following equivalent forms:
\begin{align}
\hat{\theta}[k+1]& = \beta[k] \theta[k] + (1-\beta[k]) \hat{\theta}[k] \nonumber \\
 & = \hat{\theta}[k]+\beta[k] e_{\theta}[k] \label{eq:smoothing-model}\\
 & = \sum_{t=1}^k \beta[k](1-\beta[k])^{k-t} \theta[k] \nonumber
\end{align}
where $e_{\theta}[k]:=\theta[k]-\hat{\theta}[k]$, and $\beta[k] \in (\beta_{\min},\beta_{\max}) \subset (0,1)$, is the smoothing parameter. 

\kscomment{
\begin{remark}
\label{rem:BWE-lipschitz}
Implementation of \eqref{eq:smoothing-model} requires B-agents to have access to $\theta[k]$. 
\end{remark}
}



==> lit-review.tex <==
\section{Literature Review}








==> notations.tex <==
\section{Notations}
Let $(n):=\{1,\ldots,n\}$ be the set of integers from 1 thru $n$.
